Machine learning a manifold

We propose a simple method to identify a continuous Lie algebra symmetry in a dataset through regression by an artificial neural network. Our proposal takes advantage of the $ \mathcal{O}(\epsilon^2)$ scaling of the output variable under infinitesimal symmetry transformations on the input variables. As symmetry transformations are generated post-training, the methodology does not rely on sampling of the full representation space or binning of the dataset, and the possibility of false identification is minimised. We demonstrate our method in the SU(3)-symmetric (non-) linear $\Sigma$ model.

==> universalnewcommands.tex <==
\newcommand{\half}{\frac{1}{2}}
\newcommand{\gsim}{\gtrsim}
\newcommand{\lsim}{\lesssim}
\newcommand{\ra}{\rightarrow}
\newcommand{\mtop}{m_t}
\newcommand{\ct}{c_\theta}
\newcommand{\st}{s_\theta}
\def\sigmaveeave{\langle \sigma v\rangle}
\def\sigmaveeann{\langle \sigma_{\rm ann} v\rangle}
\def\relabund{\Omega_\chi h^2}
\def\lag{\mathcal{L}}
\def\Oc{\mathcal{O}}
\def\Mc{\mathcal{M}}
\def\shat{\sqrt{\hat{s}}}
\def\shatsq{\sqrt{s}}
\def\met{\slashed{E}_T}
\newcommand{\acro}[1]{\textsc{\MakeLowercase{#1}}} %FOR `NOT SHOUTING' CAPS (e.g. acronyms)
\newcommand{\osn}{\oldstylenums}
\renewcommand{\tilde}{\widetilde} 
  % tilde over characters


\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}



\DeclareMathOperator{\ev}{eV} \DeclareMathOperator{\kev}{keV} \DeclareMathOperator{\mev}{MeV} \DeclareMathOperator{\gev}{GeV} \DeclareMathOperator{\tev}{TeV} \DeclareMathOperator{\cm}{cm} \DeclareMathOperator{\barn}{barn} \DeclareMathOperator{\km}{km} \DeclareMathOperator{\pb}{pb} \DeclareMathOperator{\s}{s} \DeclareMathOperator{\yr}{yr}\DeclareMathOperator{\gyr}{Gyr} \DeclareMathOperator{\kg}{kg} \DeclareMathOperator{\mpc}{Mpc} \DeclareMathOperator{\few}{few} \DeclareMathOperator{\kel}{K}
\newcommand{\cA}{{\cal A}} \newcommand{\cD}{{\cal D}} \newcommand{\cF}{{ \cal F}} \newcommand{\cH}{{\cal H}} \newcommand{\cJ}{{\cal J}} \newcommand{\cL}{{\cal L}} \newcommand{\cM}{{\cal M}} \newcommand{\cN}{{\cal N}} \newcommand{\cO}{{\cal O}} \newcommand{\cP}{{ \cal P}} \newcommand{\cQ}{{ \cal Q}} \newcommand{\cR}{{\cal R}} \newcommand{\cS}{{\cal S}}
\newcommand{\ep}{\epsilon} \newcommand{\vp}{\varphi}
\newcommand{\ie}{{\it i.e.}}  \newcommand{\eg}{{\it e.g.}}
\newcommand{\pt}{\partial} \def\d{{\rm d}}  \def\oL{\overline}
\newcommand{\pL}{\left(} \newcommand{\pR}{\right)} \newcommand{\bL}{\left[} \newcommand{\bR}{\right]} \newcommand{\cbL}{\left\{} \newcommand{\cbR}{\right\}} \newcommand{\mL}{\left|} \newcommand{\mR}{\right|}
\newcommand{\alg}[1]{\begin{align} \begin{split} #1 \end{split}  \end{align}}



\newcommand{\refjnl}[1]{{\rm#1}}

\def\aj{\refjnl{AJ}}                   % Astronomical Journal
\def\actaa{\refjnl{Acta Astron.}}      % Acta Astronomica
\def\araa{\refjnl{ARA\&A}}             % Annual Review of Astron and Astrophys
\def\apj{\refjnl{ApJ}}                 % Astrophysical Journal
\def\apjl{\refjnl{ApJ}}                % Astrophysical Journal, Letters
\def\apjs{\refjnl{ApJS}}               % Astrophysical Journal, Supplement
\def\ao{\refjnl{Appl.~Opt.}}           % Applied Optics
\def\apss{\refjnl{Ap\&SS}}             % Astrophysics and Space Science
\def\aap{\refjnl{A\&A}}                % Astronomy and Astrophysics
\def\aapr{\refjnl{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\def\aaps{\refjnl{A\&AS}}              % Astronomy and Astrophysics, Supplement
\def\azh{\refjnl{AZh}}                 % Astronomicheskii Zhurnal
\def\baas{\refjnl{BAAS}}               % Bulletin of the AAS
\def\bac{\refjnl{Bull. astr. Inst. Czechosl.}}
                % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{\refjnl{Chinese Astron. Astrophys.}}
                % Chinese Astronomy and Astrophysics
\def\cjaa{\refjnl{Chinese J. Astron. Astrophys.}}
                % Chinese Journal of Astronomy and Astrophysics
\def\icarus{\refjnl{Icarus}}           % Icarus
\def\jcap{\refjnl{J. Cosmology Astropart. Phys.}}
                % Journal of Cosmology and Astroparticle Physics
\def\jrasc{\refjnl{JRASC}}             % Journal of the RAS of Canada
\def\memras{\refjnl{MmRAS}}            % Memoirs of the RAS
\def\mnras{\refjnl{MNRAS}}             % Monthly Notices of the RAS
\def\na{\refjnl{New A}}                % New Astronomy
\def\nar{\refjnl{New A Rev.}}          % New Astronomy Review
\def\pra{\refjnl{Phys.~Rev.~A}}        % Physical Review A: General Physics
\def\prb{\refjnl{Phys.~Rev.~B}}        % Physical Review B: Solid State
\def\prc{\refjnl{Phys.~Rev.~C}}        % Physical Review C
\def\prd{\refjnl{Phys.~Rev.~D}}        % Physical Review D
\def\pre{\refjnl{Phys.~Rev.~E}}        % Physical Review E
\def\prl{\refjnl{Phys.~Rev.~Lett.}}    % Physical Review Letters
\def\pasa{\refjnl{PASA}}               % Publications of the Astron. Soc. of Australia
\def\pasp{\refjnl{PASP}}               % Publications of the ASP
\def\pasj{\refjnl{PASJ}}               % Publications of the ASJ
\def\rmxaa{\refjnl{Rev. Mexicana Astron. Astrofis.}}%
                % Revista Mexicana de Astronomia y Astrofisica
\def\qjras{\refjnl{QJRAS}}             % Quarterly Journal of the RAS
\def\skytel{\refjnl{S\&T}}             % Sky and Telescope
\def\solphys{\refjnl{Sol.~Phys.}}      % Solar Physics
\def\sovast{\refjnl{Soviet~Ast.}}      % Soviet Astronomy
\def\ssr{\refjnl{Space~Sci.~Rev.}}     % Space Science Reviews
\def\zap{\refjnl{ZAp}}                 % Zeitschrift fuer Astrophysik
\def\nat{\refjnl{Nature}}              % Nature
\def\iaucirc{\refjnl{IAU~Circ.}}       % IAU Cirulars
\def\aplett{\refjnl{Astrophys.~Lett.}} % Astrophysics Letters
\def\apspr{\refjnl{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\def\bain{\refjnl{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\def\fcp{\refjnl{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\def\gca{\refjnl{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\def\grl{\refjnl{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\def\jcp{\refjnl{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\def\jgr{\refjnl{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\def\jqsrt{\refjnl{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\def\memsai{\refjnl{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\def\nphysa{\refjnl{Nucl.~Phys.~A}}   % Nuclear Physics A
\def\physrep{\refjnl{Phys.~Rep.}}   % Physics Reports
\def\physscr{\refjnl{Phys.~Scr}}   % Physica Scripta
\def\planss{\refjnl{Planet.~Space~Sci.}}   % Planetary Space Science
\def\procspie{\refjnl{Proc.~SPIE}}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

